Advancing the Landscape of Multimessenger Science in the Next Decade

The last decade has brought about a profound transformation in multimessenger science. Ten years ago, facilities had been built or were under construction that would eventually discover the nature of objects in our universe could be detected through multiple messengers. Nonetheless, multimessenger science was hardly more than a dream. The rewards for our foresight were finally realized through IceCube's discovery of the diffuse astrophysical neutrino flux, the first observation of gravitational waves by LIGO, and the first joint detections in gravitational waves and photons and in neutrinos and photons. Today we live in the dawn of the multimessenger era. The successes of the multimessenger campaigns of the last decade have pushed multimessenger science to the forefront of priority science areas in both the particle physics and the astrophysics communities. Multimessenger science provides new methods of testing fundamental theories about the nature of matter and energy, particularly in conditions that are not reproducible on Earth. This white paper will present the science and facilities that will provide opportunities for the particle physics community renew its commitment and maintain its leadership in multimessenger science.

==> 260LIV-Castillo.tex <==
\vspace{0.4in}


\noindent
 \chapterauthor[1]{David Alvarez-Castillo}\orcidlink{0000-0003-1874-8116}
 \chapterauthor[]{for the CREDO Collaboration}
 \\
 \begin{affils}
    \chapteraffil[1]{Institute of Nuclear Physics PAN, Cracow 31-342, Poland}
 \end{affils}
 %dalvarez@ifj.edu.pl

The above statements underline the critical importance of the search for ultra-high-energy (UHE) photons. The project \textit{``GrailQuest:hunting for Atoms of Space and Time hidden in the wrinkle of Space–Time''} will monitor the sky in order to study astrophysical phenomena associated to such high energies utilizing nano, micro, and small satellites aiming at probing the structure of space-time~\cite{GrailQuest:2019ood}. Therefore, it will be clear that detecting delayed photons of different energies, possibly from prompt emissions of gamma-ray bursts, will serve to study deviations from the canonical dispersion relation of light in vacuo. Similarly on Earth, the \textit{Cosmic-Ray Extremely Distributed Observatory} (CREDO)~\cite{CREDO:2020pzy}, which is a global system of cosmic-ray detectors consisting mostly of smartphones, has the potential to study the arrival of photons at the ground level. CREDO seeks to incorporate detections at a wide range of scales, from terrestrial to cosmological. Figure~\ref{footprint} shows a simulation of a typical footprint of an air shower at the ground level of space-time correlated photons, often called a \textit{cosmic-ray ensemble}; see Refs.~\citenum{Dhital:2018auo,Alvarez-Castillo:2021avz} for details. Evidently, both GrailQuest and CREDO rely on large distances for photon detection. Moreover, these observatories can also take advantage of the multi-messenger approach which incorporates electromagnetic and gravitational counterparts for improved determination of the location of the photon source in case of transient events.

\begin{figure}[htpb!]
\centering
\includegraphics[width=1.0\textwidth]{260LIV-Castillo}
\caption{Cosmic-ray ensemble footprint derived from simulation. In this particular case, a primary UHE photon interacts with the magnetic field of the Sun creating an extended cosmic-ray shower. The characteristic particle distribution shows that most of the particles lie along the horizontal axis away from the central, dense core; see Refs.~\citenum{Dhital:2018auo,Alvarez-Castillo:2021avz}. Space-time resolved detections of footprints can potentially reveal a signature of Lorentz Invariance Violation.
\label{footprint}}
\end{figure}

==> 522SSDC-Gianluca_summarized_rev.tex <==
\chapterauthor[ ]{ }%not a mistake... do not remove
\vspace{-0.2in}
%adding the first few authors to table of contents with et al.
 \addtocontents{toc}{%\hspace{50pt}
     \leftskip3cm
     %\relax
%    \rightskip1cm\relax
    \scshape\small
    \parbox{5in}{\raggedleft Gianluca Polenta et al. on behalf of the SSDC staff}
    \upshape\normalsize
    \string\par
    \raggedright
    \vskip -0.19in
    % \rightskip0cm\relax
    %\leftskip0cm\relax
    }
 
 %manually adding section authors and affiliations without placing in the table
\noindent
\nocontentsline\chapterauthor[]{Gianluca Polenta$^{1}$}\orcidlink{0000-0003-4067-9196}
\nocontentsline\chapterauthor[]{Stefano Ciprini$^{1,2}$}
\nocontentsline\chapterauthor[]{Valerio D'Elia$^{1}$}
\nocontentsline\chapterauthor[]{Dario Gasparrini$^{1,2}$}\orcidlink{0000-0002-5064-9495}
\nocontentsline\chapterauthor[]{Marco Giardino$^{1}$}
\nocontentsline\chapterauthor[]{Cristina Leto$^{1}$}
\nocontentsline\chapterauthor[]{Fabrizio Lucarelli$^{1,3}$}
\nocontentsline\chapterauthor[]{Alessandro Maselli$^{1,3}$}\orcidlink{0000-0003-3760-1910}
\nocontentsline\chapterauthor[]{Matteo Perri$^{1,3}$}
\nocontentsline\chapterauthor[]{Carlotta Pittori$^{1,3}$}\orcidlink{0000-0001-6661-9779}
\nocontentsline\chapterauthor[]{Francesco Verrecchia$^{1,3}$}
\nocontentsline\chapterauthor[]{on behalf of the SSDC staff}
\\
 \begin{affils}
   \chapteraffil[1]{Space Science Data Center, Italian Space Agency, via del Politecnico snc, 00133, Roma, Italy}
   \chapteraffil[2]{INFN-Sezione di Roma Tor Vergata, 00133, Roma, Italy}
   \chapteraffil[3]{INAF-OAR, via Frascati 33, 00078 Monte Porzio Catone (RM), Italy}
\end{affils}


%\noindent
%\chapterauthor[1]{Gianluca Polenta}
%\chapterauthor[1,2]{Stefano Ciprini}
%\chapterauthor[1]{Valerio D'Elia}
%\chapterauthor[1,2]{Dario Gasparrini}
%\chapterauthor[1]{Marco Giardino}
%\chapterauthor[1]{Cristina Leto}
%\chapterauthor[1,3]{Fabrizio Lucarelli}
%\chapterauthor[1,3]{Alessandro Maselli}
%\chapterauthor[1,3]{Matteo Perri}
%\chapterauthor[1,3]{Carlotta Pittori}
%\chapterauthor[1,3]{Francesco Verrecchia}
%\chapterauthor[]{and the SSDC staff}
%\\
%\begin{affils}
%    \chapteraffil[1]{Space Science Data Center, Italian Space Agency, via del Politecnico snc, 00133, Roma, Italy}
%    \chapteraffil[2]{INFN-Sezione di Roma Tor Vergata, 00133, Roma, Italy}
%    \chapteraffil[3]{INAF-OAR, via Frascati 33, 00078 Monte Porzio Catone (RM), Italy}
%\end{affils}

%\subsection{Space Science Data Center}

{\color{blue}

The Space Science Data Center\footnote{https://www.ssdc.asi.it} (SSDC) of the Italian Space Agency (ASI) is a collaborative effort with National Institute for Astrophysics (INAF), and National Institute for Nuclear Physics (INFN), to provide a Research Infrastructure designed to facilitate collection, reduction, analysis, and distribution of data from supported science missions. The SSDC aims to develop a user-friendly, online, and public set of tools and services which fulfil the open science FAIR ({\it Findable, Accessible, Interoperable, and Reusable}) principles. 

These principles allow for non-expert users to easily navigate the large diversity of data which SSDC hosts: photon data from radio to $\gamma$-rays, as well as cosmic ray and neutrino data. This is a crucial feature for practitioners of multi-wavelength and multi-messenger science to be effective. This point is best illustrated by the tools and services available on our web portal, including: the Sky Explorer\footnote{https://tools.ssdc.asi.it}, the Multi-Mission Interactive Archive\footnote{https://www.ssdc.asi.it/mma.html}, the SSDC Data Explorer, the SED Builder\footnote{https://tools.ssdc.asi.it/SED/}, the AGILE-LV3 tool\footnote{https://www.ssdc.asi.it/mmia/index.php?mission=agilelv3mmia}, and the Fermi Online Data Analysis\footnote{https://tools.ssdc.asi.it/fermi.jsp}. Below we provide a brief description of these tools and services. A more detailed description can be found in ``The Future of Gamma-Ray Experiments in the MeVÐEeV Range'' White Paper \cite{GammaRayWP}.

The Sky Explorer is the main gateway to access SSDC services, and allows users to easily investigate an astrophysical source via SSDC's web tools simply by specifying its name or coordinates. The SSDC Multi-Mission Interactive Archive (MMIA) allows users to easily access SSDC's resident astrophysics database, which contains extensive multi-wavelength data from several space missions (e.g. AGILE, %\fermi
Fermi, Swift, NuSTAR, Herschel), and interface with other SSDC web tools. The SSDC Data Explorer, for instance, enables users to easily visualize and analyze MMIA data. Similarly, the SED Builder builds and displays the spectral energy distributions (SEDs) of astrophysical sources in the MMIA. Finally, for $\gamma$-ray data above 100 MeV, the AGILE-LV3 and the Fermi Online Data Analysis tools allow users to easily access data from AGILE and Fermi which may require substantial analysis time and to interface query results with other SSDC tools. 

}


%The Space Science Data Center\footnote{https://www.ssdc.asi.it} (SSDC) is a Research Infrastructure of the Italian Space Agency designed to acquire, reduce, analyse, and distribute data from supported science missions following the open science FAIR ({\it Findable, Accessable, Interoperable, and Reusable}) principles.

%The SSDC is all but a simple data repository. In a collaborative effort between ASI, National Institute for Astrophysics (INAF), and National Institute for Nuclear Physics (INFN), the SSDC develops online, user-friendly, publicly available scientific tools and services to allow researchers as well as non-expert users to effectively search, retrieve and use science data, thus removing those barriers possibly restricting the science exploitation to domain experts only.

%This is an important aspect in general, but it becomes crucial when addressing science topics requiring multi-wavelength and multi-messenger analysis. Indeed, the SSDC is an intrinsic multi-wavelength, multi-messenger facility hosting data from space missions covering a broad range of frequency, from radio to $\g$-ray, and different messengers (photons, cosmic rays, and neutrinos). To better illustrate this point, in the following we will highlight some of the multi-wavelength, multi-mission tools available on our web portal.

%\subsubsection{The Sky Explorer}

%The SSDC {\em Sky Explorer}\footnote{https://tools.ssdc.asi.it} represents the main access gateway to SSDC services.
%Users can specify the name, or corresponding coordinates, of their favourite astrophysical source to investigate in greater details using SSDC web tools.
%Since 2021, a new graphic layout enables the users to perform queries also for list of sources.
%The new interface, that appears after the upload of the input file, allows to manage this list in a smart way, opening simultaneously new dedicated browser tabs for each source, to start further investigations with more specific SSDC web tools such as the {\em Data Explorer} and {\em SED Builder}, simplifying the quick comparison of the obtained results.

%\subsubsection{The Multi-Mission Interactive Archive}

%The SSDC {\em Multi-Mission Interactive Archive}\footnote{https://www.ssdc.asi.it/mma.html} (MMIA) is a web-based high-energy astrophysics archive and advanced database system, which provides access to extensive multi-wavelength information. 
%Data from all SSDC resident archives can be obtained and visualized remotely in a simple and homogeneous way. 
%Through the MMIA system, archival data from several space missions (e.g. AGILE, \fermi, Swift, NuSTAR, Herschel) can be easily explored and retrieved. 
%In addition, the data can be analyzed on-line in an interactive way via various graphical web interfaces developed at the SSDC.
%With just one click, these data can enrich the collection of those retrieved from the literature and can be readily exploited in other SSDC web tools, such as the {\em SED Builder}.


%\subsubsection{The Data Explorer}
%The SSDC {\em Data Explorer} 
%is a web-based tool designed to visualize and analyze the data stored in the Multi-Mission Interactive Archive. 
%It allows the fast visualization of a portion of the sky centered on a specific source in all the energy bands, and the cross-matching between archival catalogs. 
%It also points to external services for more extended searches as well as to internal tools to perform a more detailed analysis.


%\subsubsection{The SED Builder}

%The {\em SED Builder}\footnote{https://tools.ssdc.asi.it/SED/} is a tool developed at the SSDC to build and display the Spectral Energy Distribution (SED) of astrophysical sources.

%The majority of the data comes from a large and increasing number of catalogs, extracted from ground- and space-based missions and experiments covering the whole electromagnetic spectrum, from radio to TeV energies. These include resident catalogs built with major contributions from SSDC researchers and staff, but also resources imported from external archives, such as NED, CDS, etc. The collection of input catalogs is being expanded to include the contribution of multi-messenger events, such as neutrinos and cosmic rays, that will play an increasingly large role in the forthcoming years, enabling the creation of a so-called hybrid SED.

%In addition, the {\em SED Builder} allows users to further enrich the SED for the sources of interest by adding their own datasets, as well as those resulting from recent observations of Swift, NuSTAR, AGILE and Fermi high-energy missions not included in any catalog yet. To this purpose, dedicated tools for the online analysis of these data have been developed and can be easily accessed through the SSDC web portal. Registered users are also allowed to store their datasets and SED collection.

%A key point, at variance with other tools and resources, is that SED data available in our tool are science ready. This means that infrared, optical, and ultraviolet data from all catalogs are properly corrected for Galactic dust extinction, while data in the soft X-ray energy range are corrected for Galactic absorption. Concerning catalogs from high-energy missions that are generally provided in the form of count rates, the conversion to fluxes in physical units is performed taking into account the instrument response and assuming, as a first step, a power law spectral model.

%The {\em SED Builder} provides several plotting options as well as features to analyze SED properties to fulfill userês requirements. In the first place, the choice of several flux units vs frequency, energy or wavelength to express the SEDs. Rest-frame luminosity is also allowed provided that a cosmological redshift is available, and to this purpose a photometric redshift calculator is also present. Then, the SED can be compared with templates taken from literature for various astrophysical sources, such as quasars, elliptical and spiral galaxies. Analytical functions as well as profiles resulting from numerical models, can be fitted to data to compare SEDs with theoretical expectations. Sensitivity curves of selected instruments can be overlapped to the plot, a particularly useful option for weak or undetected sources.

%The growing number of telescopes operating on a very wide range of frequencies, both ground- and space-based, increases the probability for many astrophysical sources of being repeatedly observed over time. Hence, the SED Builder allows time filtering of data in order to build time-resolved SEDs, thus making variability studies far easier, also offering the possibility to display and compare light curves at different wavelengths. In Fig.~\ref{fig:SEDMKN421}, we show a time resolved SED for MKN421 in which we adopted different colours to distinguish observations taken at different epochs tracing high and low states.

%\begin{figure}
%    \centering
%    \includegraphics[height=10cm]{SSDC-Gianluca-1}
%    \caption{Time-resolved SED for MKN421 in which different colours are used to represent data collected at different epochs in order to highlight soft X-ray variability.}
%    \label{fig:SEDMKN421}
%\end{figure}


%\subsubsection{The AGILE-LV3 tool}
%In the case of $\gamma$-rays in the energy range above 100 MeV, as for missions such as AGILE \cite{Tavani2009} and \fermi \cite{Atwood2009}, the scientific data analysis over long time-scales may require long processing times (of the order of many hours).

%\begin{figure}
%    \centering
%    \includegraphics[height=13cm,angle=0]{SSDC-GianLuca-2}
%    \caption{Combined image for illustrative purposes of hands-on data analysis with the AGILE-LV3 and SED SSDC tools.}
%    \label{fig:AGILE-LV3}
%\end{figure}

%To speed up the AGILE-GRID scientific analysis, a complete level-3 (LV3) archive of pre-compiled exposure, counts and diffuse background maps over 1-day integration time, with fixed standard parameters was created at SSDC.
%The AGILE-LV3 legacy archive can be used as basis for scientific Maximum Likelihood analysis on time scales that may vary from weeks to months, or even over the entire duration of the mission.
%For an easy AGILE-GRID official data analysis, with waiting times ranging from a few seconds to a few minutes, the interested user may query the entire public LV3 archive through the AGILE-LV3 web tool\footnote{https://www.ssdc.asi.it/mmia/index.php?mission=agilelv3mmia} \cite{Lucarelli2020}.
%In the query page the user can enter the source name or sky coordinates of the object he/she wants to analyze, the period of interest and the duration of the LV3 maps (e.g. 1, 7 or 28 days timebins) to be used in the analysis.
%The output from the query automatically selects all AGILE available observations of the source, and the $\gamma$-ray light curve over the selected period can be directly generated, see Fig.~\ref{fig:AGILE-LV3}. 

%The AGILE-LV3 tool is meant to be easily comprehensible, does not require any install-on-premises software or calibrations, and it has been even tested with high-school students. It is also directly interfaced with the SED builder and other SSDC tools.

%\subsubsection{Fermi Online Data Analysis}

%SSDC is hosting an official mirror archive of the \fermi-LAT high level data products, thus allowing to link \fermi-LAT data to SSDC tools.

%The {\it Fermi Online Data 
%Analysis}\footnote{https://tools.ssdc.asi.it/fermi.jsp} (FODA) is designed to retrieve the data in a very similar way like NASA \fermi Science Support Center, with the advantage of allowing for a quick-look analysis of the requested data as well as the analysis of science ready data for the requested region using the standard tools of the \fermi-LAT collaboration.

%Through a user-friendly web interface, the user can provide source name or sky coordinates, time interval, and energy of the interested region in order to submit the query to the archive. Given the characteristic of \fermi sky observations, it is not possible to use pre-computed products to speed up the computation, so we implemented an asynchronous query mechanism that notify the user by email of the successful completion and the availability of data for download.
%A GTLIKE analysis can also be requested, and in that case a second email will be delivered announcing that the standard analysis is completed.

%Among the results available for a given source, there are the significance of the detection during the requested periods, spectral parameters, confidence regions and high energy photons statistically associated to the requested source that could trigger TeV telescope observations. A PNG plot of the SED is also created for a quick analysis, while the resulting data point can be easily loaded into the SSDC {\em SED Builder}.


==> zz-notes.tex <==
\begin{comment}
SWGO/HAWC - Kristi Engel, Pat Harding, Andrea Albert, Jordan Goodman, Brenda Dingus, Marcos Santander (SWGO only)

CTA - David Williams (at least as POC), Marcos Santander

IceCube - Justin Vanderbrouke, Naoko Neilsen, Segev BenZvi

ARIANNA-200(?) - Steven Barwick %https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF0-NF10_NF4_S._Barwick-013.pdf

AMEGO/AMEGO-X - Carolyn Kierans, Michela Negro

COSI (w/n the current or "imminent" landscape) - Carolyn Kierans, Brenda Dingus(?)

Fermi - Michela Negro

GECCO(?) - Alexander Moiseev, Stefano Profumo
%https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF3_CF1_Stefano_Profumo-007.pdf

Auger/TA - Jaime Alvarez-Muniz

RNO-G - Stephanie Wissel

GCOS - Jorg Horandel

GRAND -  Mauricio Bustamante

POEMMA - Angela Olinto, Fred Sarazin
%https://www.snowmass21.org/docs/files/summaries/CF/SNOWMASS21-CF7_CF6-031.pdf

ZAP - Andres Romero-Wolf?

BEACON - Stephanie Wissel

PUEO - Abigail Vieregg

LIGO \& LISA -?

Synopsis: Provide short blurbs of facilities to be included here and point to other WPs.

Radar Echo Telescope?



AMON

SNEWS2.0 - Alec Habig, Rafael Lang

WEBT (Whole Earth Blazar Telescope)

Event Horizon Telescope

\end{comment}
